Data-driven prediction of vortex-induced vibration response of marine risers subjected to three-dimensional current

Slender marine structures such as deep-water marine risers are subjected to currents and will normally experience Vortex Induced Vibrations (VIV), which can cause fast accumulation of fatigue damage. The ocean current is often three-dimensional (3D), i.e., the direction and magnitude of the current vary throughout the water column. Today, semi-empirical tools are used by the industry to predict VIV induced fatigue on risers. The load model and hydrodynamic parameters in present VIV prediction tools are developed based on two-dimensional (2D) flow conditions, as it is challenging to consider the effect of 3D flow along the risers. Accordingly, the current profiles must be purposely made 2D during the design process, which leads to significant uncertainty in the prediction results. Further, due to the limitations in the laboratory, VIV model tests are mostly carried out under 2D flow conditions and thus little experimental data exist to document VIV response of riser subjected to varying directions of the current. However, a few experiments have been conducted with 3D current. We have used results from one of these experiments to investigate how well 1) traditional and 2) an alternative method based on a data driven prediction can describe VIV in 3D currents. Data driven modelling is particularly suited for complicated problems with many parameters and non-linear relationships. We have applied a data clustering algorithm to the experimental 3D flow data in order to identify measurable parameters that can influence responses. The riser responses are grouped based on their statistical characteristics, which relate to the direction of the flow. Furthermore we fit a random forest regression model to the measured VIV response and compare its performance with the predictions of existing VIV prediction tools (VIVANA-FD).

==> Paper 2 - Data driven prediction of vortex induced vibration response subjected to three-dimensional current/referee.tex <==


In any case, the proceedings will be published after the symposium and we’ll come back with instructions once the agreement with Springer is finished. In order to prepare your camera ready copy (CRC), please take the review remarks into consideration and revise your paper accordingly.

In order to be included in the proceedings, you must submit your CRC by May 20th and at least one author must register for the NAIS symposium. The paper must not exceed 12 pages (including references). As part of the final submission, we ask you also to upload your work on Arxiv and send us the Arxiv ID and the link of the paper.

Thank you for your contributions and we are looking forward to seeing you here in Trondheim!












We would like to thank both referees for useful and constructive comments, most of which have now been implemented in the paper. A few more comments are provided inline below.
----------------------- REVIEW 1 ---------------------
SUBMISSION: 2
TITLE: Data-driven prediction of vortex-induced vibration response of marine risers subjected to three-dimensional current
AUTHORS: Signe Riemer-Sørensen, Jie Wu, Halvor Lie, Svein Sævik and Sang-Woo Kim

----------- Originality of the work -----------
SCORE: 5 (excellent)
----------- Overall evaluation -----------
SCORE: 3 (strong accept)
----- TEXT:
Highly interesting, well-written and clear paper on using data-driven methods to understand and model the effects of VIV.

I only have a few comments on things that could be clarified further to make it even easier for the reader to follow:
- In Fig. 2 (and in the table of features), define the direction of the x- and y-axis.
REPLY: Done
- In Fig. 3, explain the orange vertical line in the caption.
REPLY: Done
- FFT was used to remove high frequency noise before double integration to find displacement from acceleration. Was the filtered frequency signal transformed back to time domain before integrating, or was integration performed in frequency domain?
REPLY: Integrated in frequency domain. Has been clarified in the text.
- The definitions of U, U_tot and u_tot could be more clear.
REPLY: We have added a definition of U and u_tot and removed U_tot and |u| from the notation
- In Section 3, it says "we limited the total sensor velocity to a narrow range". Does that mean that you only considered data points where the sensor measurement was in that range?
REPLY: Yes. Has been clarified in the text
- Same section: Clustering was performed on all features, and the results were used (in combination with domain knowledge) to select a subset of features for further consideration. How was the clustering used to determine the importance of individual features?
REPLY: Their importance and their correlation, in addition to visual inspection of the cluster members. Has been clarified in the text.
----------- Presentation Type -----------
SCORE: 1 (Oral Presentation)



----------------------- REVIEW 2 ---------------------
SUBMISSION: 2
TITLE: Data-driven prediction of vortex-induced vibration response of marine risers subjected to three-dimensional current
AUTHORS: Signe Riemer-Sørensen, Jie Wu, Halvor Lie, Svein Sævik and Sang-Woo Kim

----------- Originality of the work -----------
SCORE: 4 (good)
----------- Overall evaluation -----------
SCORE: 2 (accept)
----- TEXT:
This paper applies machine learning technique, both supervised and unsupervised, to marine research. A number of features were extracted from the 3D flows. First hierarchical density based clustering (HDBSCAN) was employed to identify the flow groups. Next Random Forest was used to predict the vibration response. The proposed data-driven method are significantly superior to a previous model based on differential equations in terms of accuracy. Overall the work is interesting and promising.

Below are some technical comments

1) Clustering is based a certain similarity metric. Please clarify which similarity metric was used in Section 3.
REPLY: Done
2) HDBSCAN requires two hyper-parameters: the minimal cluster size and the radius of neighborhood. Please clarify the choice of the two parameters (including the default values if used).
REPLY: Done
3) Please elaborate the split of training and testing samples. Are the cases shuffled? Is the split based on uniform sampling?
REPLY: As stated in the paper we assume the time series chunks to be independent of each other and only characterised by their statistics. The training and test data are randomly chosen from these. The assumption is justified by visual inspection of the time series and small systematic variation of their statistical parameters.
4) Especially, did you use future cases to predict the current response? If yes, the result is only valid for interpolation and it would be better to show the extrapolation results.
REPLY: The assumption of time series chunks being independent of each other means there are no "past"/"future" cases in the model fit and predictions. Apart from the acceleration and deceleration phases that we exclude, the vibration patters are fairly stable as a function of time
5) It is better to quantify the advantage over VIVANA-FD.
REPLY: Done, we have provided the root mean squared errors relative to the sensor locations for both models.
6) It is also better to show the regression results for each cluster.
REPLY: That would require three separate figures which we do not have space for in the paper, and hence we are showing an example from the most complicated scenario to show that the random forest model is superior when the assumptions of VIVANA are not fulfilled. As stated in the paper, none of the models are perfect, and ideally we will be able to merge them to a hybrid solution.

The writing is good. It would be better to separate the panels in Figure 4. Now the subplots are too small and hard to see in the printed version.
REPLY: Thanks! The font sizes have been increased on all figures, and we have removed two columns from figure 4 in order to increase the size of all examples. 
----------- Presentation Type -----------
SCORE: 2 (Poster Presentation)




==> referee.tex <==


In any case, the proceedings will be published after the symposium and we’ll come back with instructions once the agreement with Springer is finished. In order to prepare your camera ready copy (CRC), please take the review remarks into consideration and revise your paper accordingly.

In order to be included in the proceedings, you must submit your CRC by May 20th and at least one author must register for the NAIS symposium. The paper must not exceed 12 pages (including references). As part of the final submission, we ask you also to upload your work on Arxiv and send us the Arxiv ID and the link of the paper.

Thank you for your contributions and we are looking forward to seeing you here in Trondheim!












We would like to thank both referees for useful and constructive comments, most of which have now been implemented in the paper. A few more comments are provided inline below.
----------------------- REVIEW 1 ---------------------
SUBMISSION: 2
TITLE: Data-driven prediction of vortex-induced vibration response of marine risers subjected to three-dimensional current
AUTHORS: Signe Riemer-Sørensen, Jie Wu, Halvor Lie, Svein Sævik and Sang-Woo Kim

----------- Originality of the work -----------
SCORE: 5 (excellent)
----------- Overall evaluation -----------
SCORE: 3 (strong accept)
----- TEXT:
Highly interesting, well-written and clear paper on using data-driven methods to understand and model the effects of VIV.

I only have a few comments on things that could be clarified further to make it even easier for the reader to follow:
- In Fig. 2 (and in the table of features), define the direction of the x- and y-axis.
REPLY: Done
- In Fig. 3, explain the orange vertical line in the caption.
REPLY: Done
- FFT was used to remove high frequency noise before double integration to find displacement from acceleration. Was the filtered frequency signal transformed back to time domain before integrating, or was integration performed in frequency domain?
REPLY: Integrated in frequency domain. Has been clarified in the text.
- The definitions of U, U_tot and u_tot could be more clear.
REPLY: We have added a definition of U and u_tot and removed U_tot and |u| from the notation
- In Section 3, it says "we limited the total sensor velocity to a narrow range". Does that mean that you only considered data points where the sensor measurement was in that range?
REPLY: Yes. Has been clarified in the text
- Same section: Clustering was performed on all features, and the results were used (in combination with domain knowledge) to select a subset of features for further consideration. How was the clustering used to determine the importance of individual features?
REPLY: Their importance and their correlation, in addition to visual inspection of the cluster members. Has been clarified in the text.
----------- Presentation Type -----------
SCORE: 1 (Oral Presentation)



----------------------- REVIEW 2 ---------------------
SUBMISSION: 2
TITLE: Data-driven prediction of vortex-induced vibration response of marine risers subjected to three-dimensional current
AUTHORS: Signe Riemer-Sørensen, Jie Wu, Halvor Lie, Svein Sævik and Sang-Woo Kim

----------- Originality of the work -----------
SCORE: 4 (good)
----------- Overall evaluation -----------
SCORE: 2 (accept)
----- TEXT:
This paper applies machine learning technique, both supervised and unsupervised, to marine research. A number of features were extracted from the 3D flows. First hierarchical density based clustering (HDBSCAN) was employed to identify the flow groups. Next Random Forest was used to predict the vibration response. The proposed data-driven method are significantly superior to a previous model based on differential equations in terms of accuracy. Overall the work is interesting and promising.

Below are some technical comments

1) Clustering is based a certain similarity metric. Please clarify which similarity metric was used in Section 3.
REPLY: Done
2) HDBSCAN requires two hyper-parameters: the minimal cluster size and the radius of neighborhood. Please clarify the choice of the two parameters (including the default values if used).
REPLY: Done
3) Please elaborate the split of training and testing samples. Are the cases shuffled? Is the split based on uniform sampling?
REPLY: As stated in the paper we assume the time series chunks to be independent of each other and only characterised by their statistics. The training and test data are randomly chosen from these. The assumption is justified by visual inspection of the time series and small systematic variation of their statistical parameters.
4) Especially, did you use future cases to predict the current response? If yes, the result is only valid for interpolation and it would be better to show the extrapolation results.
REPLY: The assumption of time series chunks being independent of each other means there are no "past"/"future" cases in the model fit and predictions. Apart from the acceleration and deceleration phases that we exclude, the vibration patters are fairly stable as a function of time
5) It is better to quantify the advantage over VIVANA-FD.
REPLY: Done, we have provided the root mean squared errors relative to the sensor locations for both models.
6) It is also better to show the regression results for each cluster.
REPLY: That would require three separate figures which we do not have space for in the paper, and hence we are showing an example from the most complicated scenario to show that the random forest model is superior when the assumptions of VIVANA are not fulfilled. As stated in the paper, none of the models are perfect, and ideally we will be able to merge them to a hybrid solution.

The writing is good. It would be better to separate the panels in Figure 4. Now the subplots are too small and hard to see in the printed version.
REPLY: Thanks! The font sizes have been increased on all figures, and we have removed two columns from figure 4 in order to increase the size of all examples. 
----------- Presentation Type -----------
SCORE: 2 (Poster Presentation)



